3D Dynamic Point Cloud Denoising via Spatial-Temporal Graph Learning

The prevalence of accessible depth sensing and 3D laser scanning techniques has enabled the convenient acquisition of 3D dynamic point clouds, which provide efficient representation of arbitrarily-shaped objects in motion. Nevertheless, dynamic point clouds are often perturbed by noise due to hardware, software or other causes. While a plethora of methods have been proposed for static point cloud denoising, few efforts are made for the denoising of dynamic point clouds with varying number of irregularly-sampled points in each frame. In this paper, we represent dynamic point clouds naturally on graphs and address the denoising problem by inferring the underlying graph via spatio-temporal graph learning, exploiting both the intra-frame similarity and inter-frame consistency. Firstly, assuming the availability of a relevant feature vector per node, we pose spatial-temporal graph learning as optimizing a Mahalanobis distance metric $\mathbf{M}$, which is formulated as the minimization of graph Laplacian regularizer. Secondly, to ease the optimization of the symmetric and positive definite metric matrix $\mathbf{M}$, we decompose it into $\mathbf{M}=\mathbf{R}^{\top}\mathbf{R}$ and solve $\mathbf{R}$ instead via proximal gradient. Finally, based on the spatial-temporal graph learning, we formulate dynamic point cloud denoising as the joint optimization of the desired point cloud and underlying spatio-temporal graph, which leverages both intra-frame affinities and inter-frame consistency and is solved via alternating minimization. Experimental results show that the proposed method significantly outperforms independent denoising of each frame from state-of-the-art static point cloud denoising approaches.

==> algorithm.tex <==
As demonstrated in Fig.~\ref{fig:flowchart}, for a given dynamic point cloud, we perform denoising on each frame sequentially. The proposed algorithm consists of four major steps: 1) patch construction, in which we form overlapped patches from chosen patch centers; 2) similar/corresponding patch search, in which we search similar patches for each patch in the current frame, and search the corresponding patch in the previous frame; 3) graph construction, in which we build a spatio-temporal graph with intra-connectivities among similar patches and inter-connectivities among corresponding patches; 4) optimization, in which we solve the proposed problem formulation in Eq.~(\ref{eq:final_2}) via alternating minimization, thus performing step 2-4 iteratively. Note that, the inter-frame reference is bypassed for denoising the first frame as there is no previous frame. We discuss the four steps separately in detail. 


% \subsection{(to do)Similar/Corresponding Patch Search}
% \label{section:Similar/Corresponding Patch Search}
% For each constructed patch in $\hat{\mathbf{U}}_t$, we search for its similar patches locally in $\hat{\mathbf{U}}_t$, and its corresponding patch in $\hat{\mathbf{U}}_{t-1}$. A metric is necessary to measure the similarity between patches. It remains a challenging problem as the patches are irregular. 

% \textbf{Similarity Metric.}
% % truncated Chebyshev polynomial expansion
% % \begin{equation}
% % \mathbf{y} = g_\theta(\mathcal{L}) \mathbf{x} 
% %           = \sum_{k=0}^{K-1}\theta_kT_k(\mathcal{L}) \mathbf{x},
% % \label{eq:chebyshev}
% % \end{equation}
% % where $\theta_k$ denotes the $ k $-th Chebyshev coefficient. $T_k(\mathcal{L})$ is the Chebyshev polynomial of order $ k $. It is recurrently calculated by $ T_k(\mathcal{L}) = 2\mathcal{L}T_{k-1}(\mathcal{L}) - T_{k-2}(\mathcal{L})$, where $T_0(\mathcal{L}) = 1,T_1(\mathcal{L}) = \mathcal{L}$. Now the computational complexity is reduced to $ \mathcal{O}(K | \mathcal{E} | ) $.  
% We deploy a simplified method of \cite{zeng20183d} to measure the similarity between patch $\hat{\mathbf{p}}_{t,n}$ and patch $\hat{\mathbf{p}}_{t,m}$. The key idea is to compare the distance of the two patches, from each point to the tangent plane at the patch center.

% Firstly, we structure the tangent planes of the two patches. A point cloud describes the surface of the object. We thus calculate the surface normals $ \vec {n}_n $ and $\vec{n}_m $ for patch $\hat{\mathbf {p}}_ {t,n} $ and patch $ \hat{\mathbf{p}} _ {t, m } $ respectively. Then we acquire the tangent planes of the patches at the patch center $\mathbf {c} _ {t,n} $ and $ \mathbf {c} _ {t,m} $.

% Secondly, we measure the difference of patches with the distance of the two patches from each point to the corresponding tangent plane. Specifically, we project each point in patch $ \hat{\mathbf {p}} _ {t,n} $ and patch $ \hat{\mathbf{p}} _ {t,m} $ to the tangent plane of patch $ \hat{\mathbf {p}} _ {t , n } $. For the $i$-th point $\mathbf{v}_{n}^i$ in patch $ \hat{\mathbf {p}} _ {t , n } $, we find the point $\mathbf{v}_{m}^i$ in  $\hat{\mathbf {p}} _ {t , m } $, whose projection on the tangent plane is closest to that of $\mathbf{v}_{n}^i$. We then define $d_n(\mathbf{v}_n^i)$ and $d_n(\mathbf{v}_m^i)$ as the distance of the two points to their projections on the tangent plane. $|d_n(\mathbf{v}_n^i) - d_n(\mathbf{v}_m^i)|$ is regarded as the difference of the two patches in point $\mathbf{v}_n^i$ and $\mathbf{v}_m^i$. Then we acquire the average difference between the two patches at all the $(k+1)$ points:
% \begin{equation}
%     \mathbf{D}_{\overrightharp{mn}} = \sqrt{\frac{1}{k+1}\sum_{i=1}^{k+1}\left[d_n(\mathbf{v}_n^i) - d_n(\mathbf{v}_m^i)\right]^2}.
% \end{equation}
% Similarly, projecting each point in patch $\hat{\mathbf{p}}_{t,n}$ and patch $\hat{\mathbf{p}}_{t,m}$ to the tangent plane of patch $\hat{\mathbf{p}}_{t,m}$, we acquire an average difference $\mathbf{D}_{\overrightharp{nm}}$.
% The final mean difference between the two patches is:
% \begin{equation}
%     \mathbf{D}_{mn} = \sqrt{\frac{1}{2}(\mathbf{D}_{\overrightharp{mn}}^2+\mathbf{D}_{\overrightharp{nm}}^2)}.
% \end{equation}

% Finally, we measure the patch similarity with a thresholded Gaussian function using the above mean difference:
% \begin{equation}
%     \mathbf{s}_{mn} = 
%     \begin{cases}
%     \text{exp} \left( -\frac{\mathbf{D}_{mn}^2}{2\epsilon^2} \right), & \mathbf{D}_{mn}\leqslant r,\\
%     0, & \mathbf{D}_{mn} > r,
%     \end{cases}
%     \label{eq:similarity}
% \end{equation}
% where $r$ is a threshold determined by the density of the point cloud, and $\epsilon$ is a variance-related parameter.
% The larger $ \mathbf{s}_{mn}$ is, the more similar $ \hat{\mathbf {p}} _ {t,n} $ and $ \hat{\mathbf{p}} _ {t,m} $ are.  

% \textbf{Local Patch Search.} Given the similarity measure, we search for similar patches within the current frame. The number of the similar patches depends on the size of the point cloud. As to the corresponding patch in the previous frame, we only search one patch as the corresponding patch. Given a target patch in the $t$-th frame $\hat{\mathbf{p}}_{t, l}, l\in \left[1, M\right]$, we choose the most similar patch to $\hat{\mathbf{p}}_{t, l}$ in the $(t-1)$-th frame as the corresponding patch $\hat{\mathbf{p}}_{t-1, l}$. 

% In order to reduce the computation complexity, we set a local window in the $(t-1)$-th frame for the corresponding patch search, which contains patches centering at the K-nearest neighbors of the target patch center. Thus we evaluate the patch similarity between the target patch and these K-nearest patches instead of all the patches in the $(t-1)$-th frame. Once we acquire the patch $\hat{\mathbf{p}}_{t-1, l}$, we deploy its similarity measure in Eq.~(\ref{eq:similarity}) to the patch $\hat{\mathbf{p}}_{t, l}$ as the weighting parameter $w_i$ in Eq.~(\ref{eq:likelihood1}). Similarly, we set a local window for similar patch search in the $t$-th frame.

% %To keep the continuity of frames, we consider the frame $t$ and frame $t-1$. For every patch $\mathbf{p}_{m,t}$ in frame $t$, we find a corresponding patch in frame $t-1$, which is the most similar patch $\mathbf{p}_{m, t-1}'$ in frame $t-1$ of $\mathbf{p}_{m,t}$ (we will show our method to measure the similarity of patches in section 4.1).We connect the points in similar patches of frame $t$, and the points in  corresponding patches between frame $t$ and frame $t-1$ , so we get a graph connected the patches in frame $t$ and the patches in frame $t-1$. 

% \vspace{-0.1in}


\subsection{Optimization of $\mathbf{L}_t$}
This leads to the following formulation:
\begin{equation}
\begin{split}
&\min_{\mathbf{R}}
    \sum_{\{i,j\}}\exp\left\{-\|\mathbf{R} (\mathbf{f}_i - \mathbf{f}_j)\|_2^2 \right\} \, d_{i,j}\\
& \text{s.t.} \quad \,\text{tr}(\mathbf{R}) \leq C.
\label{eq:optimize_linear}
\end{split}
\end{equation}

\textbf{Frank-Wolfe Algorithm} While we can solve \eqref{eq:optimize_linear} via a proximal gradient approach, we employ the projection-free Frank-Wolfe algorithm and solve the following:
\begin{equation}
 \begin{split}
&\min_{\mathbf{R}^l}
    {\mathbf{R}^l}^{\top} \bigtriangledown F(\mathbf{n}^l)  \\
& \text{s.t.} \quad \,\text{tr}(\mathbf{R}^l) \leq C.
\label{eq:fw}
\end{split}   
\end{equation}

The linear constraint of $\mathbf{R}^l$ forms a set:
\begin{equation}
    \mathcal{S}=\left\{ \mathbf{R}^l ~\bigg|~ \text{tr}(\mathbf{R}^l) \leq C \right\}.
\end{equation}

$\bigtriangledown F(\mathbf{n}^l)$ denotes the gradient of $F(\mathbf{n}^l)=\sum_{\{i,j\}}\exp\left\{-\|\mathbf{n}^l (\mathbf{f}_i - \mathbf{f}_j)\|_2^2 \right\} \, d_{i,j}$ with respect to $\mathbf{n}^l$:
\begin{equation}
\bigtriangledown F(\mathbf{n}^l)=
-\sum_{\{i,j\}}2 (\mathbf{f}_i - \mathbf{f}_j)^{\top} \mathbf{n}^l (\mathbf{f}_i - \mathbf{f}_j)\exp\left\{-\|\mathbf{n}^l (\mathbf{f}_i - \mathbf{f}_j)\|_2^2 \right\} \, d_{i,j}
\end{equation}  

We then update the variable as
\begin{equation}
    \mathbf{n}^{l+1}=\mathbf{n}^l+\gamma(\mathbf{R}^l-\mathbf{n}^l),
\end{equation}
where $\gamma = l/(l+2)$. The linear program \eqref{eq:fw} is iteratively solved till convergence. 

% We now rewrite the optimization for $\mathbf{P}$ as an unconstrained problem by incorporating the indicator function $I_{\mathcal{S}}(\mathbf{P})$ into the objective: 
% \begin{equation}
% \min_{\mathbf{P}}
%     \sum_{\{i,j\}}\exp\left\{-\|\mathbf{P} (\mathbf{f}_i - \mathbf{f}_j)\|_2^2 \right\} \, d_{i,j} + I_{\mathcal{S}}(\mathbf{P}).
%     \label{eq:solve_P}
% \end{equation}  
% The first term is convex with respect to $\mathbf{P}$ and differentiable, while the second term $I_{\mathcal{S}}(\mathbf{P})$ is convex but non-differentiable. 
% we can thus employ PG to solve (\ref{eq:solve_P}) as follows. 


% We next define a proximal mapping $\Pi_{I_{\mathcal{S}}}(\mathbf{v})$ for the second term---indicator function $I_{\mathcal{S}}(\mathbf{v})$---which is a projection onto the linear set $\mathcal{S}$, i.e.,
% \begin{equation}
%     \Pi_{I_{\mathcal{S}}}(\mathbf{v})=
%     \left\{
%         \begin{array}{lr} 
%             \mathbf{v} & \text{tr}(\mathbf{P}) \leq C,  \\
%             \mathbf{v}-\alpha\cdot\vec{1}, & \text{otherwise,}
%         \end{array}
%     \right.
% \end{equation}
% where $\alpha$ is any positive root of $\vec{1}^{\top}(\mathbf{v}-\alpha\cdot\vec{1}) = C$ \cite{beck2017first}.

% Each iteration of the PG algorithm can be now written as:
% \begin{equation}
%     \mathbf{P}^{l+1}=\Pi_{I_{\mathcal{S}}}(\mathbf{P}^{l}-t\bigtriangledown F(\mathbf{P}^{l})),
% \end{equation}
% where $t$ is the step size.

\subsection{Optimization of $\mathbf{W}_{t,t-1}$}
\begin{equation} 
\begin{split}
&\min_{\mathbf{W}_{t, t-1}} \mathbf{W}_{t,t-1}\| (\mathbf{S}_{t}\mathbf{U}_{t} - \mathbf{C}_{t}) - \hat{\mathbf{P}}_{t-1} \|_2^2.\\
& 
% \label{E4}
\end{split}
\label{eq:final_3}
\end{equation} 

Combining the Mahalanobis distance, we have 
\begin{equation}
\begin{split}
&\min_{\mathbf{R}}
    \sum_{\{i,j\}}\exp\left\{-\|\mathbf{R} (\mathbf{f}_i - \mathbf{f}_j)\|_2^2 \right\} \, \tilde{d}_{i,j}\\
& \text{s.t.} \quad \,\text{tr}(\mathbf{R}) \leq C.
\label{eq:optimize_linear}
\end{split}
\end{equation}
where $\tilde{d}_{i,j}$ denotes the squared Euclidean distance between the coordinates of temporally corresponding points. 

Similar to the optimization of $\mathbf{L}_t$, we employ the Frank-Wolfe algorithm to iteratively solve $\mathbf{R}$ and finally compute $\mathbf{W}_{t,t-1}$ from the Gaussian kernel in \eqref{eq:weight}. 

In this section, we elaborate on the proposed problem formulation. We start from the modeling of a dynamic point cloud sequence via spatio-temporal GMRFs, and propose such modeling on patch basis. Then we pose a MAP estimation of the underlying dynamic point cloud, and come up with the likelihood function and prior distribution. Finally, we arrive at the problem formulation from the MAP estimation.   

\vspace{-0.1in}

\begin{algorithm}[htb]
  \caption{3D Dynamic Point Cloud Denoising}  
  \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
  \label{alg:Framwork}
    \Input{A noisy dynamic point cloud sequence $\hat{\mathcal{P}}=\{\hat{\mathbf{U}}_1,\hat{\mathbf{U}}_2,...,\hat{\mathbf{U}}_m\}$} 
    \Output{Denoised dynamic point cloud sequence  $\mathcal{P}=\{\mathbf{U}_1,\mathbf{U}_2,...,\mathbf{U}_m\}$} 
    \For{$\hat{\mathbf{U}}_t$ in $\hat{\mathcal{P}}$}{
        Initialize $\mathbf{U}_t$ with $\hat{\mathbf{U}}_t$ \\
        Select $M$ points (set $\mathbf{C}_t$) as patch centers; \\
        \For{$\mathbf{c}_l$ in $\mathbf{C}_t$}{
            Find $k$-nearest neighbors of $\mathbf{c}_l$; \\
            Build patch $\hat{\mathbf{p}}_{t,l}$; \\
            Add $\hat{\mathbf{p}}_{t,l}$ to $\hat{\mathbf{P}}_t$; \\
        }
            \Repeat{convergence}{
            \For{$\hat{\mathbf{p}}_{t,l}$ in $\hat{\mathbf{P}}_t$}{
                \For {$\hat{\mathbf{p}}_{t, j}$ in $\hat{\mathbf{p}}_{t,l}$'s adjacent patches}{
                    Calculate the similarity metric $s_{l, j}$ between $\hat{\mathbf{p}}_{t,l}$ and $\hat{\mathbf{p}}_{t, j}$ as in Eq.~(\ref{eq:similarity}); \\
                    Connect nearest points in $\hat{\mathbf{p}}_{t,l}$ and $\hat{\mathbf{p}}_{t, j}$ with the edge weight $s_{l, j}$; \\
                }
                Search the corresponding patch $\hat{\mathbf{p}}_{t-1,l}$ of $\hat{\mathbf{p}}_{t,l}$ in the previous frame, which is the most similar to $\hat{\mathbf{p}}_{t,l}$ in terms of the metric metric $s_{(t-1)l, tl}$ as in Eq.~(\ref{eq:similarity}); \\
                Connect corresponding points in $\hat{\mathbf{p}}_{t,l}$ and $\hat{\mathbf{p}}_{t-1, l}$ with the edge weight $s_{(t-1)l, tl}$; \\
            }
            Compute the intra-frame graph Laplacian $\mathbf{L}_t$; \\
            Compute the weight matrix $\mathbf{W}_{t,t-1}$ between corresponding patches; \\
            Solve Eq.~(\ref{eq:closed_form_U}) to update $\mathbf{U}_t$; \\
        }
        $\mathbf{U}_t$ serves as the input for the denoising of the next frame.
    }
\end{algorithm}  





==> old_formulation.tex <==

\subsection{Spatial-Temporal Modeling}
A dynamic point cloud sequence $\mathcal{P}=\{\mathbf{U}_1,\mathbf{U}_2,...,\mathbf{U}_m\}$ consists of $m$ frames of point clouds. The coordinates $\mathbf{U}_t=[\mathbf{u}_{t,1}, \mathbf{u}_{t,2}, ... , \mathbf{u}_{t,n}]^\top\in \mathbb{R}^{n\times3}$ denote the position of each point in the point cloud at frame $t$, in which $\mathbf{u}_{t,i} \in \mathbb{R}^3$ represents the coordinates of the $i$-th point at frame $t$. Let $\mathbf{U}_t$ denote the ground truth coordinates of the $t$-th frame, and $\hat{\mathbf{U}}_{t-1}$, $\hat{\mathbf{U}}_t$ denote the noise-corrupted coordinates of the $(t-1)$-th and $t$-th frame respectively. Then we formulate the dynamic point cloud denoising problem as
\begin{equation}
    \hat{\mathbf{U}}_t = f(\mathbf{U}_{t-1},\mathbf{U}_t) + \mathbf{E}_t,
    \label{eq:model}
\end{equation}
where $\mathbf{E}_t \in \mathbb{R}^{n\times3}$ is a zero-mean signal-independent noise. For point clouds acquired from equipments, the noise distribution is related to the acquisition equipments. Several previous works \cite{nguyen12, xiafang08} have shown through statistics that the noise in point clouds approximates Gaussian distribution for 3D scanning equipments such as Microsoft Kinect, 3D laser scanner, etc. As these are popular sensors, we assume the noise follows Gaussian distribution. 

\textbf{Spatio-temporal GMRF modeling.} In particular, we model the relationship in consecutive frames of a dynamic point cloud via spatio-temporal GMRF models. A spatial GMRF is a restrictive multivariate Gaussian distribution that satisfies additional conditional independence assumptions. A graph is often used to represent the conditional independence assumption. Here is the formal definition:

\textbf{Definition:} A random vector $\vec{x} = (x_1, x_2, ..., x_n)^\top \in \mathbb{R}^n$ is a GMRF with respect to a graph $\mathcal{G}=\{\mathcal{V},\mathcal{E}\}$ with mean $\mu$ and precision matrix $\mathbf{Q} > 0$, if its density has the form
\begin{equation}
    \pi(\vec{x}) = (2\pi)^{-\frac{n}{2}}|\mathbf{Q}|^{\frac{1}{2}} \text{exp}\left(-\frac{1}{2}(\vec{x}-\vec{\mu})^\top\mathbf{Q}(\vec{x}-\vec{\mu})\right),
    \label{eq:gmrf}
\end{equation}
and
\begin{equation}
    Q_{i,j} \neq 0 \quad \Longleftrightarrow \quad \{i,j\} \in \mathcal{E}, \forall i \neq j.
\end{equation}

Spatio-temporal GMRF models are extensions of spatial GMRF models to account for additional temporal variation. In our case, we represent a dynamic point cloud of $m$ frames on a sequence of $m$ subgraphs. Each subgraph describes the \textit{intra-frame connectivities} within each frame, and temporal connectivities exist between neighboring subgraphs to describe the \textit{inter-frame connectivities}.    

\textbf{Patch representation.} Further, as it is computationally expensive to consume  an  entire point cloud, we model both intra-frame and inter-frame dependencies on \textit{patch} basis. Unlike images or videos defined on regular grids, point clouds reside on irregular domain with uncertain local neighborhood, thus the definition of a patch is nontrivial. We define a patch $\mathbf{p}_{t,l} \in \mathbb{R}^{(k+1) \times 3}$ in the point cloud at frame $t$ as a local point set of $k+1$ points, consisting of a centering point $\mathbf{c}_{t,l} \in \mathbb{R}^3$ and its $k$-nearest neighbors in terms of Euclidean distance. Then the entire set of patches at frame $t$ is     
\begin{equation}
    \mathbf{P}_t = \mathbf{S}_t \mathbf{U}_t-\mathbf{C}_t,
    \label{eq:patch}
\end{equation}
where $\mathbf{S}_t\in\{0, 1\}^{(k+1)M\times n}$ is a sampling matrix to select points from point cloud $\mathbf{U}_t$ so as to form $M$ patches of $(k+1)$ points each, and $\mathbf{C} \in \mathbb{R}^{(k+1)M\times 3}$ contains the coordinates of patch centers for each point.

Based on the patch representation, we model the intra-frame dependency by building graph connectivities among \textit{similar patches} within a frame, and model the inter-frame dependency by constructing graph connectivities between \textit{corresponding patches} over consecutive frames. The details of searching similar patches within a frame and corresponding patches between frames will be discussed in section \ref{section:Similar/Corresponding Patch Search}.  

 \begin{figure*}
    \includegraphics[width=\linewidth]{flowchart.pdf}
    \caption{The flowchart of the proposed dynamic point cloud denoising algorithm.}
    \label{fig:flowchart}
\end{figure*}

\vspace{-0.1in}
\subsection{MAP Estimation of Dynamic Point Clouds}
Under the spatio-temporal GMRF modeling, we pose a MAP estimation for the underlying patches $\mathbf{P}_t$ in the point cloud $\mathbf{U}_t$ at frame $t$: given the observed noisy previous frame $\hat{\mathbf{P}}_{t-1}$ and current noisy frame $\hat{\mathbf{P}}_t$, find the most probable signal $\mathbf{P}_t$,   
\begin{equation}
    \mathbf{P}_t^\text{MAP}(\hat{\mathbf{P}}_{t-1},\hat{\mathbf{P}}_t) = \argmax_{\mathbf{P}_t}  f(\hat{\mathbf{P}}_{t-1},\hat{\mathbf{P}}_t \mid \mathbf{P}_t)g(\mathbf{P}_t),
    \label{eq:map}
\end{equation}
where $f(\hat{\mathbf{P}}_{t-1},\hat{\mathbf{P}}_t \mid \mathbf{P}_t)$ is the likelihood function, and $g(\mathbf{P}_t)$ is the signal prior. Because $\mathbf{P}_t$ are patches that cover the entire $\mathbf{U}_t$, Eq.~(\ref{eq:map}) also gives the MAP estimation of $\mathbf{U}_t$:
 \begin{equation}
     \mathbf{U}_t^\text{MAP}(\hat{\mathbf{P}}_{t-1},\hat{\mathbf{P}}_t) = \argmax_{\mathbf{U}_t}  f(\hat{\mathbf{P}}_{t-1},\hat{\mathbf{P}}_t \mid \mathbf{P}_t)g(\mathbf{P}_t).
     \label{eq:mapU}
 \end{equation}

\textbf{The proposed likelihood function.} $f(\hat{\mathbf{P}}_{t-1},\hat{\mathbf{P}}_t \mid \mathbf{P}_t)$ is the probability of obtaining the observed point clouds $\hat{\mathbf{P}}_{t-1}$ and $\hat{\mathbf{P}}_t$ given the desired current frame $\mathbf{P}_t$. We have
\begin{equation}
\begin{split}
    f(\hat{\mathbf{P}}_{t-1},\hat{\mathbf{P}}_t \mid \mathbf{P}_t) = &f(\hat{\mathbf{P}}_{t-1}\mid \mathbf{P}_t, \hat{\mathbf{P}}_t) f(\hat{\mathbf{P}}_t\mid\mathbf{P}_t) \\ = & f(\hat{\mathbf{P}}_{t-1}\mid \mathbf{P}_t)f(\hat{\mathbf{P}}_t\mid\mathbf{P}_t), 
\end{split}
\label{eq:likelihood}
\end{equation}
where $f(\hat{\mathbf{P}}_{t-1}\mid \mathbf{P}_t, \hat{\mathbf{P}}_t) $ is equivalent to $f(\hat{\mathbf{P}}_{t-1}\mid \mathbf{P}_t) $ because we assume the noise of the $(t-1)$-th frame and $t$-th frame are independent.

For the second term in Eq.~(\ref{eq:likelihood}), according to the linear relationship of $\mathbf{P}_t$ and $\mathbf{U}_t$ as in Eq.~(\ref{eq:patch}) and assuming zero-mean Gaussian distribution for the noise, we have
\begin{equation}
\begin{split}
\argmax_{\mathbf{U}_t}f(\hat{\mathbf{P}}_t\mid \mathbf{P}_t) &=\argmax_{\mathbf{U}_t}f(\hat{\mathbf{U}}_t\mid \mathbf{U}_t) \\ &=\argmax_{\mathbf{U}_t}f(\hat{\mathbf{U}}_t - \mathbf{U}_t\mid \mathbf{U}_t) \\ &=\argmax_{\mathbf{U}_t}\alpha_1 \text{exp} \left(-\lambda_1\left\|\hat{\mathbf{U}}_t-\mathbf{U}_t\right\|_2^2 \right),
\end{split}
\label{eq:likelihood2}
\end{equation}
where $\alpha_1$ is a normalization factor to keep the integral of the probability function equal to 1, and $\lambda_1$ is a variance-related parameter. 

For the first term in Eq.~(\ref{eq:likelihood}), since the variation between adjacent frames is often trivial, we assume the current frame is a perturbed version of the previous frame. In particular, we propose to adopt a weighting parameter $w_i$ to represent the perturbation at the $i$-th patch, leading to  
\begin{equation}
\begin{split} 
f(\hat{\mathbf{P}}_{t-1}\mid \mathbf{P}_{t})  =  \alpha_2 \text{exp} \left(-\lambda_2 \sum_{i=1}^{M}w_i\left\|\hat{\mathbf{P}}_{t-1, i} - \mathbf{P}_{t, i}\right\|_2^2 \right), 
\end{split}
\label{eq:likelihood1}
\end{equation}
where $\alpha_2$ is a normalization factor, and $\lambda_2$ is a variance-related parameter. 
In the proposed algorithm, $w_i$ is a variable depending on $\hat{\mathbf{P}}_{t-1, i}$ and $\mathbf{P}_{t,i}$, which describes the similarity between $\hat{\mathbf{P}}_{t-1, i}$ and $\mathbf{P}_{t,i}$.   

% If $\mathbf{P}_{t-1}$ is given, assuming zero mean of noise, the conditional probability distribution of $\hat{\mathbf{P}}_{t-1}$ can be expressed as:
% \begin{equation}
% \begin{split} \label{EQ10}
% f(\hat{\mathbf{P}}_{t-1}\mid \mathbf{P}_{t-1})  = &f(\hat{\mathbf{P}}_{t-1}-\mathbf{P}_{t-1}\mid \mathbf{P}_{t-1}) \\= & \alpha_2 \text{exp} (-\lambda_2 \left\|\hat{\mathbf{P}}_{t-1} - \mathbf{P}_{t-1}\right\|_2^2) \\ = &  \alpha_2 \text{exp} (-\lambda_2 \sum_{i=1}^{M}\left\|\hat{\mathbf{P}}_{t-1, i} - \mathbf{P}_{t-1, i}\right\|_2^2)
% \end{split}
% \end{equation}
% We can't get the exact relationship of $\mathbf{P}_{t, i}$ and $\mathbf{P}_{t-1, i}$, so we build a simplified model to simplify the problem. We assume that $f(\hat{\mathbf{P}}_{t-1}\mid \mathbf{P}_t) $ have the similar form with $f(\hat{\mathbf{P}}_{t-1}\mid \mathbf{P}_{t-1}) $. We add an weighting term $w_i$ for every patch in Eq.~(\ref{EQ10}), then we get:


\textbf{The proposed prior distribution.} Since $\mathbf{U}_t$ follows GMRF modeling, assuming zero mean, we have its prior distribution from Eq.~(\ref{eq:gmrf}) as:   
\begin{equation}
    g(\mathbf{P}_t) = \beta \text{exp} \left(-\frac{1}{2}\mathbf{P}_t^\top\mathbf{Q}_t\mathbf{P}_t\right),
    \label{eq:prior_p}
\end{equation}
where $\mathbf{Q}_t$ is the precision matrix of the $t$-th frame, and $\beta$ is a normalization factor.

However, it is challenging to estimate $\mathbf{Q}_t$ statistically from small amounts of data. Instead, as introduced in \cite{zhang2014point}, the precision matrix can be interpreted by the graph Laplacian, i.e., $\mathbf{Q} = \delta \mathbf{L}$ by a scalar $\delta$. Hence, we replace $\mathbf{Q}_t$ in Eq.~(\ref{eq:prior_p}) by the graph Laplacian $\mathbf{L}_t$, leading to
\begin{equation}
    g(\mathbf{P}_t) = \beta \text{exp} \left(-\frac{1}{2}\mathbf{P}_t^\top\mathbf{L}_t\mathbf{P}_t \right).
    \label{eq:prior_p_final}
\end{equation}

\vspace{-0.1in}
\subsection{Final Problem Formulation}
Combining Eq.~(\ref{eq:mapU}), Eq.~(\ref{eq:likelihood}), Eq.~(\ref{eq:likelihood2}), Eq.~(\ref{eq:likelihood1}), Eq.~(\ref{eq:prior_p_final}), we have
\begin{equation}
\begin{split}
    & \mathbf{U}_t^\text{MAP}(\hat{\mathbf{P}}_{t-1},\hat{\mathbf{P}}_t) \\
    = \ & \argmax_{\mathbf{U}_t} \ f(\hat{\mathbf{P}}_t|\mathbf{P}_t)f(\hat{\mathbf{P}}_{t-1}|\mathbf{P}_t)g(\mathbf{P}_t) \\ 
    = \ & \argmax_{\mathbf{U}_t}\ \begin{split}  & \alpha_1 \text{exp} \left( -\lambda_1\left\|\hat{\mathbf{U}}_t-\mathbf{U}_t\right\|_2^2 \right) \\
    & \cdot \alpha_2 \text{exp} \left(-\lambda_2 \sum_{i=1}^{M}w_i\left\|\hat{\mathbf{P}}_{t-1, i} - \mathbf{P}_{t, i}\right\|_2^2 \right)\\
    & \cdot \beta \text{exp} \left(-\frac{1}{2}\mathbf{P}_t^\top\mathbf{L}_t\mathbf{P}_t \right). \end{split} \\
    % = \argmin_{\mathbf{U}_t}\  & \lambda_1||\mathbf{U}_t-\hat{\mathbf{U}}_t||_2^2 \\ &+\lambda_2\sum\limits_{i=1}^{M}{w_i||\mathbf{P}_{t,i}-\hat{\mathbf{P}}_{t-1,i}||_2^2} \\ &+\mathbf{P}_t^\top\mathbf{L}_{t}\mathbf{P}_t
    \label{eq:final_1}
    \end{split}
\end{equation}
Due to the dependency of $\mathbf{L}_t$ and $w_i$ on $\mathbf{U}_t$, $w_i$ and $\mathbf{L}_t$ are optimization variables as well as $\mathbf{U}_t$.

Taking logarithm of Eq.~(\ref{eq:final_1}) and multiplying by $-1$, we arrive at the final problem formulation:
\begin{equation}
\begin{split}
&\min\limits_{\mathbf{U}_t,\mathbf{L}_t,w_i} \lambda_1||\mathbf{U}_t-\hat{\mathbf{U}}_t||_2^2+\lambda_2\sum\limits_{i=1}^{M}{w_i||\mathbf{P}_{t,i}-\hat{\mathbf{P}}_{t-1,i}||_2^2}+\mathbf{P}_t^\top \mathbf{L}_{t}\mathbf{P}_t,\\
& \quad \text{s.t.} \quad \, \mathbf{P}_t = \mathbf{S}_t \mathbf{U}_t-\mathbf{C}_t.
\label{eq:final_2}
\end{split}
\end{equation}
As $\mathbf{U}_t$, $\mathbf{L}_t$ and $w_i$ are optimization variables, Eq.~(\ref{eq:final_2}) is nontrivial to solve. We develop an efficient algorithm to address this problem formulation in the next section. 



